Deep Learning-based Imaging in Radio Interferometry

The sparse layouts of radio interferometers result in an incomplete sampling of the sky in Fourier space which leads to artifacts in the reconstructed images. Cleaning these systematic effects is essential for the scientific use of radiointerferometric images. Established reconstruction methods are often time-consuming, require expert-knowledge, and suffer from a lack of reproducibility. We have developed a prototype Deep Learning-based method that generates reproducible images in an expedient fashion. To this end, we take advantage of the efficiency of Convolutional Neural Networks to reconstruct image data from incomplete information in Fourier space. The Neural Network architecture is inspired by super-resolution models that utilize residual blocks. Using simulated data of radio galaxies that are composed of Gaussian components we train Deep Learning models whose reconstruction capability is quantified using various measures. The reconstruction performance is evaluated on clean and noisy input data by comparing the resulting predictions with the true source images. We find that source angles and sizes are well reproduced, while the recovered fluxes show substantial scatter, albeit not worse than existing methods without fine-tuning. Finally, we propose more advanced approaches using Deep Learning that include uncertainty estimates and a concept to analyze larger images.

==> latexmkrc <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -o %D %O %S";

###############################
# Post processing of pdf file #
###############################

# assume the jobname is 'output' for sharelatex
my $ORIG_PDF_AGE = -M "output.pdf"; # get age of existing pdf if present

END {
    my $NEW_PDF_AGE = -M "output.pdf";
    return if !defined($NEW_PDF_AGE); # bail out if no pdf file
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE; # bail out if pdf was not updated
    $qpdf //= "/usr/local/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf; # check that qpdf exists
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});
    my $status = system($qpdf, split(' ', $qpdf_opts), "output.pdf", "output.pdf.opt");
    my $exitcode = ($status >> 8);
    print "qpdf exit code=$exitcode\n";
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($exitcode == 0 || $exitcode == 3);
    print "Renaming optimised file to output.pdf\n";
    rename("output.pdf.opt", "output.pdf");
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
my $root_file = $ARGV[-1];

add_cus_dep( 'Rtex', 'tex', 0, 'rtex_to_tex');
sub rtex_to_tex {
    do_knitr("$_[0].Rtex");
}

sub do_knitr {
    my $dirname = dirname $_[0];
    my $basename = basename $_[0];
    system("Rscript -e \"library('knitr'); setwd('$dirname'); knit('$basename')\"");
}

my $rtex_file = $root_file =~ s/\.tex$/.Rtex/r;
unless (-e $root_file) {
    if (-e $rtex_file) {
        do_knitr($rtex_file);
    }
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############
sub asy {return system("asy --offscreen '$_[0]'");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}


==> sections/10_additions.tex <==
% \begin{table*}
%     \sisetup{table-number-alignment = right}
%     \centering
%     \caption{Overview of the mean results of the three evaluation methods with clean, noisy and noisy plus additional white noise input images and for input images with different mask filling.}
%   \begin{tabular}{c
%   S[table-format=1.2]@{${}\pm{}$}S[table-format=1.2]
%   S[table-format=3.2]@{${}\pm{}$}S[table-format=2.2, table-number-alignment = left]
%   S[table-format=3.2]@{${}\pm{}$}S[table-format=1.2, table-number-alignment = left]
%   }
%     \toprule
%     & \multicolumn{2}{c}{Jet offset / $\si{\degree}$} & \multicolumn{2}{c}{Intensity deviation / $\si{\percent}$} & \multicolumn{2}{c}{Source area ratio} \\
%     \midrule
%     {Clean input} & 0.03 & 1.53 & 0.36 & 14.26 & 0.98 & 0.13 \\
%     {Noisy input} & -0.11 & 2.40 & 0.04 & 20.02 & 0.96 & 0.17 \\
%     {Noise \& white noise} & -0.01 &  3.17 & 1.55 & 29.29 & 0.98 & 0.23 \\
%     \toprule
%     Sampling Density \\
%     \midrule
%     \SI{20}{\percent} & -0.10 & 4.79 & -2.25 & 40.55 & 0.83 & 0.32 \\
%     \SI{50}{\percent} & -0.25 & 1.57 & -1.02 & 14.57 & 0.97 & 0.14 \\
%     \SI{70}{\percent} & -0.19 & 1.49 & -1.49 & 13.98 & 0.98 & 0.14 \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:results_conclusion_new}
% \end{table*}

% \begin{figure*}
%     \centering
%     \resizebox{\hsize}{!}
%     {\includegraphics[width=\hsize]{images/evaluation/prediction_4.png}}
%     \caption{Exemplary reconstruction of point-like Gaussian data with the model trained on noisy input data. Visualization of prediction (left), true distribution (middle) and the difference between both (right). Results are shown for amplitude (top) and phase (bottom).}
%     \label{fig:amp-phase-point}
% \end{figure*}

% \begin{figure*}
%     \centering
%     \resizebox{0.985\hsize}{!}
%     {\includegraphics[width=\hsize]{images/evaluation/fft_pred_4.png}}
%     \caption{Sky brightness reconstruction with the predicted amplitude and phase distributions. Resulting clean image (left), simulated brightness distribution (middle) and difference between both (right).}
%     \label{fig:source-recon-point}
% \end{figure*}


% \section{A\&A Improvements}

